An Eye-Tracking Dataset for Viewing Distance Categories in Real-World Scenarios

Estimating viewing distance from gaze behavior is essential for understanding user intent and enabling distance-aware interactive systems. However, most existing eye-tracking datasets have been collected in constrained settings, such as laboratory environments or static tasks. Consequently, they only partially capture viewing behaviors in real-world situations where viewing distance changes with natural head and body movements. We introduce GazeDepth, an eye-tracking dataset collected from 19 participants using a wearable tracker during tasks reflecting real-world scenarios. GazeDepth includes fixed-distance viewing scenarios with constant observer-target distances at near (33 cm), middle (50 cm), and far (300 cm), as well as variable-distance viewing scenarios in which participants shift gaze among targets at different depths in indoor and outdoor environments. The dataset provides synchronized gaze data, pupil size, 3D eye-vectors, and head-motion signals, along with distance labels. Statistical analyses showed that distance-related gaze features, such as vergence angle and estimated viewing distance, differed consistently across viewing-distance categories. In addition, classification models trained on GazeDepth further demonstrated that the dataset captures gaze characteristics that distinguish the three viewing-distance categories, supporting gaze-based distance inference and distance-aware interaction in realistic scenarios.

==> Figure/fig_structure.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1\textwidth]{Figure/Dataset_structure.pdf}
\caption{Hierarchical file structure of \dataset dataset.}
\label{fig:dataset_structure}
\end{figure}

==> Table/tab_alpha.tex <==
\begin{table}[t]
\centering
\caption{Annotation counts and inter-rater agreement for the variable-distance indoor and outdoor tasks. 
Agreement was computed using Krippendorff’s $\alpha$ based on labels from three annotators per task. 
Mean (SD) values are reported in the last row of each task block.}
\label{tab:participant_alpha_by_task}
\begin{tabular}{cccc}
\toprule
\textbf{Task} & \textbf{ParticipantID} & \textbf{Annotated frame count} & \textbf{Krippendorff’s $\alpha$} \\
\midrule
\multirow{6}{*}{\centering Variable-distance indoor}
& P1  & 2,024 & 0.9682 \\
& P9  & 3,609 & 0.9590 \\
& P11 & 2,362 & 0.9267 \\
& P13 & 2,266 & 0.9548 \\
& P15 & 2,101 & 0.9598 \\
& P19 & 2,242 & 0.9651 \\
& \textbf{Mean (SD)} & \textbf{2434 (588.20)} & \textbf{0.9556 (0.0149)} \\
\midrule
\multirow{7}{*}{\centering Variable-distance outdoor}
& P4  & 2,282 & 0.7771 \\
& P5  & 1,875 & 0.6980 \\
& P7  & 2,088 & 0.8077 \\
& P10 & 2,719 & 0.7140 \\
& P12 & 1,741 & 0.6619 \\
& P18 & 2,118 & 0.6844 \\
& \textbf{Mean (SD)} & \textbf{2137.17 (342.92)} & \textbf{0.7239 (0.0566)} \\
\bottomrule
\end{tabular}
\end{table}

==> Table/tab_autoManualCompare.tex <==
\begin{table}[t]
\centering
\caption{Concordance between automatically generated labels and manually annotated labels for each task (variable-distance indoor/outdoor). 
For each reference set (Annotator 1-3 and majority vote), values are reported as Mean (SD) across participants for Accuracy, F1 score, and valid frame count. 
Valid frame count denotes the number of frames assigned to the valid viewing-distance classes (near, middle, far).}
\label{tab:auto_vs_annotators}
\begin{tabular}{llccc}
\toprule
\textbf{Task} & \textbf{Pair (auto vs.)} & \textbf{Accuracy} & \textbf{F1-Score} & \textbf{Valid frame count} \\
\midrule
\multirow{4}{*}{Variable-distance indoor}
& annotator1 & 0.908 (0.07) & 0.886 (0.05) & 24040.33 (3512.63) \\
& annotator2 & 0.896 (0.07) & 0.861 (0.06) & 24094.50 (3476.17) \\
& annotator3 & 0.902 (0.07) & 0.877 (0.05) & 24159.67 (3466.97) \\
& majority   & 0.905 (0.07) & 0.881 (0.05) & 24079.50 (3490.49) \\
\midrule
\multirow{4}{*}{Variable-distance outdoor}
& annotator4 & 0.873 (0.05) & 0.761 (0.06) & 8750.67 (2196.67) \\
& annotator5 & 0.793 (0.05) & 0.792 (0.05) & 12583.50 (3327.47) \\
& annotator6 & 0.803 (0.04) & 0.791 (0.04) & 12236.50 (3018.23) \\
& majority   & 0.822 (0.05) & 0.810 (0.05) & 11610.83 (2932.72) \\
\bottomrule
\end{tabular}
\end{table}

==> Table/tab_calibration_error.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.12}
\caption{Angular gaze error after post-offset correction. Values are reported as mean (SD) in degrees.}
\label{tab:calibration_residual_error}
\begin{tabular}{lccccc}
\hline
\thead{\textbf{Participant}} &
\thead{\textbf{Baseline}\\\textbf{multi-object}} &
\thead{\textbf{Fixed}\\\textbf{near}} &
\thead{\textbf{Fixed}\\\textbf{middle}} &
\thead{\textbf{Fixed}\\\textbf{far}} &
\thead{\textbf{Variable}\\\textbf{indoor}} \\
\hline
P1 & 1.25 (0.48) & 0.89 (0.44) & 1.13 (0.42) & 1.46 (0.80) & 0.80 (0.27) \\
P2 & -- & 0.65 (0.32) & 1.30 (0.45) & 1.40 (0.52) & 2.66 (1.42) \\
P3 & -- & -- & -- & -- & -- \\
P4 & 0.43 (0.19) & 1.00 (0.73) & 1.65 (0.59) & 0.51 (0.24) & 1.01 (0.39) \\
P5 & 0.56 (0.33) & 0.67 (0.38) & 0.92 (0.40) & 1.68 (0.99) & 0.90 (0.55) \\
P6 & 1.06 (0.44) & 0.56 (0.36) & 1.57 (1.20) & 1.53 (0.60) & 1.23 (0.61) \\
P7 & 0.56 (0.29) & 1.08 (0.38) & 2.48 (1.02) & 0.93 (0.31) & 1.12 (0.95) \\
P8 & 0.37 (0.14) & 0.53 (0.26) & 0.54 (0.24) & 0.46 (0.14) & 0.32 (0.14) \\
P9 & 0.69 (0.37) & 1.66 (0.93) & 0.70 (0.31) & 0.76 (0.41) & 0.82 (0.35) \\
P10 & 0.36 (0.20) & 1.90 (0.42) & 0.44 (0.27) & 0.34 (0.21) & 0.33 (0.23) \\
P11 & 0.32 (0.21) & 1.43 (0.69) & 1.07 (0.51) & 0.73 (0.46) & 0.75 (0.44) \\
P12 & 0.65 (0.30) & 0.63 (0.27) & 0.82 (0.65) & 0.45 (0.24) & 0.61 (0.36) \\
P13 & 0.28 (0.15) & 1.45 (0.75) & 0.34 (0.15) & 0.96 (0.48) & 0.47 (0.19) \\
P14 & 0.40 (0.24) & 1.26 (0.33) & 0.63 (0.22) & 0.50 (0.17) & 1.78 (1.26) \\
P15 & 0.66 (0.16) & 0.62 (0.20) & 0.46 (0.24) & 0.70 (0.36) & 1.44 (0.28) \\
P16 & 0.63 (0.31) & 0.45 (0.18) & 0.37 (0.21) & 0.63 (0.36) & 2.14 (0.32) \\
P17 & 0.36 (0.14) & 0.54 (0.27) & 0.50 (0.20) & 0.74 (0.23) & 0.84 (0.42) \\
P18 & 0.37 (0.16) & 0.64 (0.31) & 0.63 (0.22) & 1.70 (0.21) & 0.81 (0.26) \\
P19 & 0.47 (0.23) & 0.85 (0.48) & 0.62 (0.22) & 1.33 (0.27) & 0.82 (0.46) \\
\hline
\end{tabular}
\end{table*}

==> Table/tab_events.tex <==

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{Event labels used in \texttt{events.csv}.}
\label{tab:event_lists}
\begin{tabularx}{\textwidth}{l l X}
\toprule
Scope & Event label & Description \\
\midrule
Global &
\texttt{recording.start / recording.end} &
Start and end of the recording. \\

Global &
\texttt{task.start / task.end} &
Start and end of the task within a recording. \\

Global &
\texttt{dot\_calibration} &
Frame used as the reference point when an additional dot-based calibration is performed. \\

Global &
\texttt{screenrecording.start} &
Start of the screen recording when the viewed screen video is available. \\
\midrule

Dot-fixating &
\texttt{dot\_n/m/f.start / dot\_n/m/f.end} &
Start and end of near (n), middle (m), and far (f) dot-fixating segments. \\

Surface-viewing &
\texttt{plain.start / plain.end} &
Start and end of the surface-viewing task. \\

Multi-object viewing &
\texttt{mscoco.start / mscoco.end} &
Onset and offset of image presentation in the multi-object viewing task. \\
\midrule

Near-distance viewing &
\texttt{reading.start / reading.end} &
Start and end of the book-reading task at near distance. \\

Mid-distance viewing &
\texttt{login.start / login.end} &
Start and end of the login task at middle distance. \\

Mid-distance viewing &
\texttt{t\{n\}.start / t\{n\}.end} &
Start and end of individual web-browsing segments, where $n = 1 \dots 14$. Participants sometimes revisited previously failed tasks after finishing the others, so earlier task numbers may reappear later. \\


Far-distance viewing &
\texttt{t\{n\}.start / t\{n\}.end} &
Start and end of far-distance object-search segments, where $n = 1 \dots 20$. \\
\midrule

Variable-distance indoor &
\texttt{t\{n\}.start / t\{n\}.end} &
Start and end of skewer-making in the board-game task, where $n = 1 \dots 39$ ($n = 0$ denotes a practice session). \\

Variable-distance outdoor &
\texttt{destination\{1,2\}.start / destination\{1,2\}.end} &
Start and end of each route segment (route 1 and route 2) in the outdoor route-finding task. \\

Variable-distance outdoor &
\texttt{t\{n\}.start / t\{n\}.end} &
Start and end of tasks given at specific locations, where $n = 1 \dots 5$. \\
\bottomrule
\end{tabularx}
\end{table}

==> Table/tab_modelResultFixed.tex <==
\begin{table}[t]
\centering
\caption{Classification performance for Near/Middle/Far distance conditions in the fixed-distance viewing task. Performance was evaluated using accuracy and F1-score across repeated runs. Values are reported as Mean (SD) across the model.}
\label{tab:model_performanceFixed}
\begin{tabular}{lcc}
\toprule
Model & Accuracy & F1-score  \\
\midrule
MLP & 91.59 (6.50) & 91.60 (6.52) \\
Decision Tree & 82.82 (10.57) & 82.76 (10.98) \\
Random Forest & 89.54 (10.65) & 89.51 (10.88) \\
kNN & 86.94 (8.20) & 86.88 (8.36) \\
LDA & 93.17 (4.21) & 93.23 (4.07) \\
XGBoost & 91.24 (8.96) & 91.17 (9.34) \\
\bottomrule
\end{tabular}
\end{table}

==> Table/tab_modelResultIndoor.tex <==
\begin{table}[t]
\centering
\caption{Classification performance for Near/Middle/Far distance conditions in the variable-distance indoor task. Performance was evaluated using accuracy and F1-score across repeated runs.  Values are reported as Mean (SD) across the model.}
\label{tab:model_performanceIndoor}
\begin{tabular}{lcc}
\toprule
Model & Accuracy  & F1-score  \\
\midrule
MLP & 81.59 (6.34) & 72.88 (6.44) \\
Decision Tree & 73.02 (5.37) & 66.03 (5.19) \\
Random Forest & 81.54 (5.66) & 71.29 (5.88) \\
kNN & 75.65 (5.39) & 63.98 (4.40) \\
LDA & 80.44 (5.64) & 71.28 (4.83) \\
XGBoost & 81.16 (6.03) & 71.92 (6.49) \\
\bottomrule
\end{tabular}
\end{table}

==> Table/tab_modelResultOutdoor.tex <==
\begin{table}[t]
\centering
\caption{Classification performance for Near/Middle/Far distance conditions in the variable-distance outdoor task. Performance was evaluated using accuracy and F1-score across repeated runs.  Values are reported as Mean (SD) across the model.}
\label{tab:model_performanceOutdoor}
\begin{tabular}{lcc}
\toprule
Model & Accuracy & F1-score \\
\midrule
MLP & 75.49 (4.70) & 65.24 (5.34) \\
Decision Tree & 64.93 (4.81) & 60.11 (3.52) \\
Random Forest & 75.73 (4.60) & 65.36 (4.65) \\
kNN & 71.29 (3.97) & 62.80 (3.62) \\
LDA & 74.09 (4.62) & 64.43 (4.09) \\
XGBoost & 75.19 (4.70) & 65.75 (4.67) \\
\bottomrule
\end{tabular}
\end{table}



==> Table/tab_statResultFixed.tex <==
\begin{table}[t]
\centering
\caption{Significant effects of viewing distance on physiological measures in the fixed-distance tasks. We report the overall test per feature and post hoc paired tests ($p<.05$). Main $p$ values are reported using thresholds. Significant pairs are abbreviated as N (Near), M (Middle), and F (Far). In the last column, pairs are grouped by $p$-value thresholds.}
\label{tab:stats_fixed}
\begin{tabular}{l l c l}
\toprule
Feature & Test & Main $p$ & Significant pairs \\
\midrule
\textbf{Distance measure} \\
Gaze distance & Friedman & $<.001$ &
N--M, N--F ($<.001$); M--F ($<.01$) \\
Vergence angle &  & $<.001$ &
N--M, N--F ($<.001$); M--F ($<.01$) \\
\midrule
\textbf{Pupil diameter} \\
Pupil diameter (L)  & Friedman & $<.001$ &
N--F, M--F ($<.01$) \\
Pupil diameter (R)  &  & $<.05$ &
M--F ($<.01$); N--F ($<.05$) \\
\midrule
\textbf{Eyeball center} \\
Eyeball center (L) $x$  & RM-ANOVA & n.s. &
N--M ($<.05$) \\
Eyeball center (L) $y$  &  & $<.001$ &
M--F ($<.001$); N--F ($<.01$) \\
Eyeball center (L) $z$  &  & $<.001$ &
N--M, N--F, M--F ($<.001$) \\
Eyeball center (R) $x$  &  & n.s. &
None \\
Eyeball center (R) $y$  &  & $<.001$ &
M--F ($<.001$); N--F ($<.01$) \\
Eyeball center (R) $z$  &  & $<.001$ &
N--M, N--F, M--F ($<.001$)\\
\midrule
\textbf{Optical axis} \\
Optical axis (L) $x$ & Friedman & $<.001$ &
N--M, N--F ($<.001$) \\
Optical axis (L) $y$ &  & $<.001$ &
N--M, N--F, M--F ($<.001$) \\
Optical axis (L) $z$ &  & $<.001$ &
N--M, N--F ($<.001$); M--F ($<.01$) \\
Optical axis (R) $x$ &  & $<.001$ &
N--F, M--F ($<.001$) \\
Optical axis (R) $y$ &  & $<.001$ &
N--M, N--F, M--F ($<.001$) \\
Optical axis (R) $z$ &  & $<.001$ &
N--F ($<.001$); N--M, M--F ($<.01$) \\
\bottomrule
\end{tabular}
\end{table}

==> Table/tab_statResultIndoor.tex <==
\begin{table}[t]
\centering
\caption{Significant effects of viewing distance on physiological measures in the variable-distance indoor task. We report the overall test per feature and post hoc paired tests ($p<.05$). Main $p$ values are reported using thresholds. Significant pairs are abbreviated as N (Near), M (Middle), and F (Far). In the last column, pairs are grouped by $p$-value thresholds.}
\label{tab:stats_indoor}
\begin{tabular}{l l c l}
\toprule
Feature & Test & Main $p$ & Significant pairs \\
\midrule
\textbf{Distance measure} \\
Gaze distance & Friedman & $<.001$ &
N--M, N--F, M--F ($<.001$) \\
Vergence angle &  & $<.001$ &
N--M, N--F, M--F ($<.001$) \\
\midrule
\textbf{Pupil diameter} \\
Pupil diameter (L)  & Friedman & $<.001$ &
N--M, N--F ($<.001$); M--F ($<.01$) \\
Pupil diameter (R)  &  & $<.001$ &
N--M, N--F ($<.001$); M--F ($<.01$) \\
\midrule
\textbf{Eyeball center} \\
Eyeball center (L) $x$  & RM-ANOVA & $<.05$ &
N--F ($<.05$) \\
Eyeball center (L) $y$  &  & $<.001$ &
N--M, N--F, M--F ($<.001$) \\
Eyeball center (L) $z$  &  & $<.001$ &
N--F ($<.001$); N--M, M--F ($<.01$) \\
Eyeball center (R) $x$  &  & $<.05$ &
N--F ($<.05$) \\
Eyeball center (R) $y$  &  & $<.001$ &
N--M, N--F, M--F ($<.001$) \\
Eyeball center (R) $z$  &  & $<.01$ &
N--F, M--F ($<.05$) \\
\midrule
\textbf{Optical axis} \\
Optical axis (L) $x$ & Friedman & n.s. & None \\
Optical axis (L) $y$ &  & $<.001$ &
N--M, N--F, M--F ($<.001$) \\
Optical axis (L) $z$ &  & $<.001$ &
N--M, N--F ($<.001$); M--F ($<.01$) \\
Optical axis (R) $x$ &  & $<.001$ &
N--M, N--F, M--F ($<.001$) \\
Optical axis (R) $y$ &  & $<.001$ &
N--M, N--F, M--F ($<.001$) \\
Optical axis (R) $z$ &  & $<.001$ &
N--M, N--F ($<.001$); M--F ($<.05$) \\
\bottomrule
\end{tabular}
\end{table}


==> Table/tab_statResultOutdoor.tex <==
\begin{table}[t]
\centering
\caption{Significant effects of viewing distance on physiological measures in the variable-distance outdoor task. We report the overall repeated-measures ANOVA per feature and \textit{uncorrected} post hoc paired $t$-tests. Main $p$ values are reported using thresholds. Significant pairs are abbreviated as N (Near), M (Middle), and F (Far). In the last column, pairs are grouped by $p$-value thresholds.}
\label{tab:stats_outdoor}
\begin{tabular}{l l c l}
\toprule
Feature & Test & Main $p$ & Significant pairs \\
\midrule
\textbf{Distance measure} \\
Gaze distance & RM-ANOVA & $<.001$ &
N--M, N--F ($<.001$); M--F ($<.05$) \\
Vergence angle &  & $<.001$ &
N--M, N--F ($<.001$); M--F ($<.01$) \\
\midrule
\textbf{Pupil diameter} \\
Pupil diameter (L)  & RM-ANOVA & n.s. & None \\
Pupil diameter (R)  &  & n.s. & None \\
\midrule
\textbf{Eyeball center} \\
Eyeball center (L) $x$  & RM-ANOVA & n.s. &
N--M ($<.05$) \\
Eyeball center (L) $y$  &  & $<.001$ &
N--F, M--F ($<.001$); N--M ($<.01$) \\
Eyeball center (L) $z$  &  & $<.01$ &
M--F ($<.001$); N--F ($<.01$) \\
Eyeball center (R) $x$  &  & $<.05$ &
N--M ($<.05$) \\
Eyeball center (R) $y$  &  & $<.001$ &
N--F, M--F ($<.001$); N--M ($<.01$) \\
Eyeball center (R) $z$  &  & $<.01$ &
M--F ($<.001$); N--F ($<.01$) \\
\midrule
\textbf{Optical axis} \\
Optical axis (L) $x$ & RM-ANOVA & $<.001$ &
N--F, M--F ($<.001$); N--M ($<.01$) \\
Optical axis (L) $y$ &  & $<.001$ &
N--M, N--F, M--F ($<.001$) \\
Optical axis (L) $z$ &  & $<.001$ &
N--M, N--F ($<.001$); M--F ($<.01$) \\
Optical axis (R) $x$ &  & $<.001$ &
N--M, N--F ($<.001$); M--F ($<.05$) \\
Optical axis (R) $y$ &  & $<.001$ &
N--M, N--F, M--F ($<.001$) \\
Optical axis (R) $z$ &  & $<.001$ &
N--M, N--F ($<.001$) \\
\bottomrule
\end{tabular}
\end{table}
